Low Rank Fusion based Transformers for Multimodal Sequences

Our senses individually work in a coordinated fashion to express our emotional intentions. In this work, we experiment with modeling modality-specific sensory signals to attend to our latent multimodal emotional intentions and vice versa expressed via low-rank multimodal fusion and multimodal transformers. The low-rank factorization of multimodal fusion amongst the modalities helps represent approximate multiplicative latent signal interactions. Motivated by the work of~\cite{tsai2019MULT} and~\cite{Liu_2018}, we present our transformer-based cross-fusion architecture without any over-parameterization of the model. The low-rank fusion helps represent the latent signal interactions while the modality-specific attention helps focus on relevant parts of the signal. We present two methods for the Multimodal Sentiment and Emotion Recognition results on CMU-MOSEI, CMU-MOSI, and IEMOCAP datasets and show that our models have lesser parameters, train faster and perform comparably to many larger fusion-based architectures.

==> intro.tex <==

\section{Introduction}



==> introduction.tex <==
Sentiment Analysis is broadly defined as the computational study of subjective elements such as opinions, attitudes, and emotions towards other objects or persons. Sentiments attach to modalities such as text, audio and video at different levels of granularity and are useful in deriving social insights about various entities such as movies, products, persons or organizations. Emotion Understanding is another closely related field that commonly deals with analysis of audio, video, and other sensory signals for getting psychological and behavioral insights about an individual's mental state. Emotions are defined as brief organically synchronized evaluations of major events whereas sentiments on the other hand are considered as more enduring beliefs and dispositions towards objects or persons \cite{scherer1984emotion}. The field of Emotion Understanding has rich literature with many interesting models of understanding \cite{plutchik2001nature} \cite{ekman2009telling} \cite{posner2005circumplex}.

In this work, we explore methods that combine various unimodal techniques for classification alongwith multimodal techniques for fusion of cross modal interactions to perform sentiment analysis and emotion understanding. We develop and test our approaches on the CMU-MOSEI dataset \cite{zadeh2016multimodal} as part of the ACL Multimodal Emotion Recognition grand challenge. CMU Multimodal Opinion Sentiment and Emotion Intensity (CMU-MOSEI) dataset is a newly released large dataset of multimodal sentiment analysis and emotion recognition on YouTube video segments. The dataset contains more than 23,500 sentence utterance videos from more than 1000 online YouTube speakers. The dataset has several interesting properties such as being gender balanced, containing various topics and monologue videos from people with different personality traits. The videos are manually transcribed and properly punctuated. Since the dataset comprises of natural audio-visual opinionated expressions of the speakers, it provides an excellent testbed for research in emotion and sentiment understanding. The videos are cut into continuous segments and the segments are annotated with 7 point scale sentiment labels and 4 point scale emotion categories corresponding to the Ekman's 6 basic emotion classes \cite{10025007347}. The opinionated expressions in the segments contain visual cues, audio variations in signal as well textual expressions showing various subtle and non-obvious interactions across the modalities for both sentiment and emotion classification.

What differentiates our work from existing literature is (i) application of a novel cross modal fusion technique across the temporal segments of the multimodal channel (ii) use of rich shallow semantic domain knowledge that include a large number of psycholinguistic features and resources for sentiment and emotion classification and (iii) extraction of emotion aware acoustic phoneme level features using a novel method and architecture.

Our unimodal research focus in this paper is an exploration of speech sentiment and emotion recognition using various text dependent and text independent techniques. On the text modality experiments, we've explored (i) fusion of Lexicons as additional input features (ii) fusion of polarity discriminating lexico-syntactic fine-grained scores as additional input features (iii) fusion of rich contextualized embeddings as additional input features to the classification pipeline. On audio modality, we've used a novel pipeline to generate the iVectors and Phoneme level utterance features. For fusion of multimodal information, we have explored techniques that leverage intra-modal and inter-modal dynamics and fused them together in a novel Relational Tensor Network architecture. 

%\begin{figure}
%\includegraphics[scale=0.4]{fusion1.png}
%\caption{Relational Tensor Network}
%    \label{arch}
%\end{figure}



==> model.tex <==
\section{Model and Architecture}
Motivated by (Zadeh et al., 2017) and (Poria et al., 2017), we present our model Relational-TFN that considers intra-segment multi-modal interactions using tensor fusion network and an LSTM based architecture to model the relations and interactions across sequence of segments in a video. 


\subsection{Text Network}

